SpeechBlender: Speech Augmentation Framework for Mispronunciation Data Generation

The lack of labeled second language (L2) speech data is a major challenge in designing mispronunciation detection models. We introduce SpeechBlender - a fine-grained data augmentation pipeline for generating mispronunciation errors to overcome such data scarcity. The SpeechBlender utilizes varieties of masks to target different regions of phonetic units, and use the mixing factors to linearly interpolate raw speech signals while augmenting pronunciation. The masks facilitate smooth blending of the signals, generating more effective samples than the `Cut/Paste' method. Our proposed technique achieves state-of-the-art results, with Speechocean762, on ASR dependent mispronunciation detection models at phoneme level, with a 2.0% gain in Pearson Correlation Coefficient (PCC) compared to the previous state-of-the-art [1]. Additionally, we demonstrate a 5.0% improvement at the phoneme level compared to our baseline. We also observed a 4.6% increase in F1-score with Arabic AraVoiceL2 testset.

==> sections/algorithm.tex <==
\begin{algorithm}[h]
\label{algo:top}
\caption{SpeechBlender function}
\SetAlgoLined
\KwIn{Input phoneme frame sequences $x_C$ and $x_D$ where $x_C = \{f^1_C \cdots f^T_C\}$ and $x_D = \{f^1_D \cdots f^L_D\}$, where ($T$, $L$) are total frames in ($x_C$, $x_D$) respectively. $y_C$ represent the original output score assigned to the good phoneme.}
\KwOut{Augmented frame output sequences $\hat{x}$ and the corresponding label $\hat{y}$ of the output.}

\SetKwFunction{FMain}{Blender}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$x_C, x_D, y_C$}}{
        $\theta_{\hat{x}} \longleftarrow [ ]$ \Comment{Store augmented output per region}
        
        $\theta_{\hat{y}} \longleftarrow [ ]$ \Comment{Store corresponding partial output score}
        
        $mid \longleftarrow rand([1,4])$ \Comment{Mask template id}
        
        $\rho \longleftarrow get\_property(mid, len(x_C), len(x_D)) $ \Comment{Mask property}
        
        $ W, \Lambda \longleftarrow generate\_mask(\rho)$ 
        % \footnote{In case of MDD, the positive class represents -- missed, mispronounced or accented phonemes, and the negative classes are good pronounced phonemes.}

        
        \Comment{$W$: list of regional mask width, $\Lambda$: list of regional mixing factor values.}\
        % \Comment{}\
        % \Comment{$\hat{y}$: Output labels depending on the mixing factor}\
        % \Comment{$R$: list of frames divided in to regions, $\Lambda$: list of mixing factor for each region, $ \hat{y}$: generated output label  }
        
        
        % \Comment{$R \in  \{1, 2, 3\}$, $\Lambda \in [0-1]$, $ \hat{y} \in \{0, 1\}$ }
        
        
        \ForEach{$ w \in W$ and $ \lambda  \in \Lambda $}
        { 
        
        
        $\theta_{\hat{x}} \longleftarrow$ $\lambda \cdot x{_C^w}$ + $(1-\lambda ) \cdot x{_D^w}$ %\Comment{sorted list by weight}
        
        $\theta_{\hat{y}} \longleftarrow \lambda \cdot y{_C}$
        }
        $\hat{x} \longleftarrow  Concat(\theta_{\hat{x}})$ %\Comment{join the regions generate augmented sample}
        
        $\hat{y} \longleftarrow   \left \lfloor \sum\theta_{\hat{y}}/len(\Lambda)\right \rfloor$
        
        
        \textbf{return} $\hat{x} , \hat{y} $ %\; 
}

\end{algorithm}
\vspace{-0.2cm}

==> sections/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

In this paper, we introduce a fine-grained data augmentation technique, SpeechBlender, and show its efficacy in generating new error classes for a phoneme-level and grapheme-level pronunciation quality detection task. The SpeechBlender linearly interpolate raw input signals using different blending masks like `\textit{SmoothOverlay}' and mixing factors $\lambda$. Varieties of masks included in the proposed method allows smooth modification in different regions of the phoneme.  
With SpeechBlender, we observe improved performance compared to \textit{(i)} no-augmentation, \textit{(ii)} multi-task learning scenario, \textit{(iii)} text-augmentation, and \textit{(iv)} GOP-augmentation setting. We noticed the \textit{`Cut/Paste'} method be it in text-, feature- or raw-audio domain, is not as efficient as the proposed interpolation technique. 



Moreover, our results suggest that with blending the signals, we can generate new positive error classes instead of reusing samples from the data itself in zero-shot setting. %, without any dependence on the error labels from the original data.
% , we are able to generate new error samples and improve the performance. 
The different choices of masks allow variations in transition and style of errors. In future, we will further explore the capability of SpeechBlender for generating accented/erroneous phoneme candidate for other speech tasks like ASR, while exploring multiple granularities.
% hus making such augmentation more 

==> sections/experimentnresult.tex <==
\section{Experiments} 
\label{sec:exp}


%In this Section, we describe the dataset and the system architectures used in our study. %to show the efficacy of the proposed SpeechBlender augmentation. 

\subsection{Speech Corpus}
Table \ref{tab:output_defination} shows details about the datasets used in our study. For English, we opted for the Speechocean$762$ \cite{speechocean}, %a free open-source dataset designed to assess the pronunciation quality of L$2$ learners. The dataset 
which consists of $5,000$ English utterances from $250$ non-native speakers with rich annotation labels. Five experts annotate each phoneme, and the final phoneme accuracy score is calculated as their average. For Arabic, we use an in-house corpus, AraVoiceL2, which is comprised of $5.5$ hours of data recorded by $11$ non-native Arabic speakers. Each speaker recorded a fixed list of $642$ words and short sentences, making for a total of $7,062$ recordings. We split AraVoiceL2 data, $7$ speakers for training and $6$ speakers for testing. %daThe training set consists of recordings from $7$ speakers, the remaining $6$ speakers recordings are used for testing. 

%For the study, we opt for the Speechocean762 \cite{speechocean}, a free open-source dataset designed to assess the pronunciation quality of L2 learners. The dataset consists of 5,000 English utterances from 250 non-native speakers with rich annotation labels. Along with different utterances and the word level quality aspects, the dataset includes accuracy scores at phoneme-level that are divided based on three class labels, as shown in Table \ref{tab:output_defination}. %Each phoneme is annotated by five experts and the final phoneme accuracy score is calculated as their average. % of all the scores.
%Five experts annotate each phoneme, and the final phoneme accuracy score is calculated as their average.

% For our study, we focus on modeling just these phoneme scores. for each phoneme, five accuracy scores were given by five expert annotators. The final phoneme accuracy score is calculated as the average or median experts scores (ranging from 0-2). The training set consists of 47246 phonemes, and distributed as follows.

% We conduct Speechocean762 dataset to evaluate the performance of our techniques, it is publicly available. Speechocean is non-native English corpus for pronunciation assessment, it consists of 250 speakers, whose L1-Language is not English. The overall dataset consists of 5000 English utterances richly labeled at the phoneme level, word level, and utterance level. In our study, we are interested in accuracy scores given at phoneme level. A pronounced phoneme is classified to 3 classes: 

\begin{table*}[!ht]
\centering
\scalebox{1.0}{
\begin{tabular}{l|c c | c c | c c } 
 \hline
%  (Avg. Scores)
  &   \multicolumn{2}{c}{\textbf{English phoneme}} & \multicolumn{2}{c}{\textbf{Arabic phoneme}}                                         &  \multicolumn{2}{c}{\textbf{Arabic grapheme}}   \\
 Label  &  Training & Testing & Training & Testing & Training & Testing \\
 \hline\hline
%  ($0<=p<0.5$)
 0     & $1,991$ & $1,339$ & $97$ & $94$ &  $95$ & $89$ \\ 
 \hline
%  ($0.5<=p<1.5$)
 1   & $1,967$ & $1,828$ & $707$ & $618$ & $590$ & $483$ \\
 \hline
%  ($p>=1.5$)
 2   & $43,118$ &  $44,079$ & $28,270$  &  $23,008$ & $20,255$  &  $16,511$ \\
 \hline
\end{tabular}
}

\caption{Phoneme-level statistics for the English corpus, and phoneme, grapheme-level statistics for the Arabic corpus, along with the score definition used in the study. Label (\textit{0}): mispronounced or missing phoneme, label (\textit{1}): accented pronunciation and label (\textit{2}): is for good pronunciation.}
\label{tab:output_defination}
\end{table*}


%\begin{table}[!ht]
%\centering
%\scalebox{0.8}{
%\begin{tabular}{l|c |c | c} 
% \hline
%  (Avg. Scores)
% Label  & Label Description & Train Set & Test Set \\
% \hline\hline
%  ($0<=p<0.5$)
% 0    & \begin{tabular}{c}
%      mispronounced or \\
%      missing phoneme
% \end{tabular}  & $97$ & $94$ \\ 
% \hline
%  ($0.5<=p<1.5$)
% 1   & accented pronunciation & $707$ & $618$  \\
% \hline
%  ($p>=1.5$)
%2   & good pronunciation & $28,270$  &  $23,008$  \\
% \hline
%\end{tabular}
%}

%\caption{Details phoneme-level statistics and score definition used %in the \textbf{Arabic} AraVoiceL2 Dataset = Phoeneme level}
%\label{tab:output_defination}
%\end{table}

%\begin{table}[!ht]
%\centering
%\scalebox{0.8}{
%\begin{tabular}{l|c |c | c} 
% \hline
%  (Avg. Scores)
% Label  & Label Description & Train Set & Test Set \\
% \hline\hline
%  ($0<=p<0.5$)
% 0    & \begin{tabular}{c}
%      mispronounced or \\
%      missing phoneme
% \end{tabular}  & 95 & 89 \\ 
% \hline
%  ($0.5<=p<1.5$)
% 1   & accented pronunciation & 590 & 483  \\
% \hline
%  ($p>=1.5$)
% 2   & good pronunciation & 20255  &  16511  \\
% \hline
%\end{tabular}
%}

%\caption{Details phoneme-level statistics and score definition used in AraVoiceL2 Dataset -Grapheme level}
%\label{tab:output_defination}
%\end{table}


% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c|c} 
%  \hline
%  Class & \# Percentage & \# Total \\
%  \hline\hline
%  0   & 3\% & 1339\\ 
%  \hline
%  1  & 4\% & 1828\\
%  \hline
%  2  & 93\% & 44079\\
%  \hline
% \end{tabular}
% \caption{Phoneme classes distribution using ceiling function of the final accuracy score }
% \label{tab:phoneme_distribution}
% \end{table}
% \subsection{System overview}
\subsection{Mispronunciation Detection Model}

% An overview of the mispronunciation detection model architecture is presented in Figure \ref{fig:architecture}.

Given the input audio and the canonical transcription, we first extract the frame-level phonetic features using pre-trained ASR, described in Section \ref{ssec:asr}. Using the acoustic model, we calculated the 84-dimensional GOP features for 42 pure phonemes. 
Each phone GOP representation contain two different features: \textit{(i)} log phone posterior (LPP) \cite{transfer_} of a phone $p$ of length $T$ frames with per frame observation $o_t$ see Equation \ref{eq:lpp}; 
% (see Equation \ref{eq:lpp})
and \textit{(ii)} the log posterior ratio (LPR) \cite{transfer_} of phone $p_{j}$ with respect to phone $p_i$, as given in Equation \ref{eq:lpr} 
\begin{equation}
\label{eq:lpp}
\begin{small}
LPP(p) = \frac{1}{T} \sum log\ p(p|o_t)
\end{small}
\end{equation}
\begin{equation}
\label{eq:lpr}
LPR(p_j|p_i) = log\ p(p_j|o_t) - log\ p(p_i|o_t)
\end{equation}
\noindent These 84-dimensional features are then passed through a feed-forward layer to project the GOP embeddings in 24 dimensional feature space.  
Simultaneously, we inject the textual-content information using the one-hot vector representation of the canonical phoneme transcription. These vector representations are then projected to 24-dimensional phoneme embedding and are then added to the GOP representations.

% \begin{figure} [!ht]
% \centering
% \vspace{-0.4cm}
% \includegraphics[scale=0.45]{figures/lstm.png}
% \vspace{-0.2cm}
% \caption{Illustration of the proposed LSTM architecture with a sample utterance “My Name”. The number of encoder layers $N=3$}
% \label{fig:architecture}
% \end{figure}

Consequently, we pass the final representation to the encoder network. As our encoder, we opt for a long short-term memory (LSTM)\footnote{Additional models such as SVR\cite{speechocean}, MLP are tested with SpeechBlender data augmentation. As the results follow the same trend , for brevity we are reporting the results using LSTM only.}
% , we observed a 3\% increase in PCC} 
network due to the model's strength in capturing preceding contextual information, and its reduced computational cost without losing much on the model accuracy. For further comparison, we implement the architecture with similar configuration as \cite{JIM} with 3 stacked LSTM layers and an output embedding dimension of 24. We then pass the embedding per phoneme to the output layer for the regression task.

\noindent\textbf{Model Parameters}: We train the mispronunciation detection model using an Adam optimizer for $50$ epochs with a starting learning rate of $1e-3$ and a batch size of $32$. The learning rate is then cut in to its half in every 3 epochs, after 10 initial epochs. 
Regarding the loss function, it is adapted to suit the specific annotations dataset. Specifically, for the English dataset, which involves a continuous task and scores ranging from 0 to 2, we have utilized the mean squared error (MSE). In contrast, for the Arabic dataset, which involves a classification task, we adopted cross entropy.

% As for the loss function, we use the mean squared error (MSE) for English, and cross entropy for Arabic. We report the results based on the last epoch.

\subsection{Evaluation Measures}
We measure the proposed models performance using standard statistical metric: 
We report MSE and PCC for the English dataset, and Precision (PR), Recall (RE), and F1-score for the Arabic Dataset. We use PCC, F1-score for ranking as they are more representative of the performance in such an imbalanced class scenario. 


\section{Results and Discussion}
%In this Section, we report the results in Table \ref{tab:results_1} with different augmentation settings and compare it with no-augmentation and multi-task learning setup proposed in \cite{JIM}. We validate our proposed augmentation pipeline using the Speechocean762 test data and Arabic Data set. Furthermore, we show the strength of each mask proposed with the SpeechBlender and compare it with the Cut/Paste method in Table \ref{tab:resuts_2}.
% We first compare the results with and without any augmentation for only phoneme-level and then compa 

\subsection{Speechocean762 dataset:}
\paragraph*{Comparison with Baselines:} We benchmark our results in Table \ref{tab:results_1}, the PCC results indicate the importance of augmentation in general. Our results indicates that Text-Augmentation, GOP-augmentation and SpeechBlender augmentation outperforms the model with only Speechocean762 trainset by $1\%$, 1$\%$, and $5\%$ respectively. 
% The GOP-augmentation, a feature space replacing technique, performs comparable with the multi-task learning setup with a PCC of $0.59$. 
Our novel augmentation technique surpassed the performance of Text-augmentation, GOP-augmentation, and the multi-task setup using LSTM\cite{JIM} model by $4$\% using only phoneme-level information for training. Furthermore, we achieved better results than the state-of-the-art reported PCC \cite{JIM}, GOP Transformer model in a multi task set-up, with an improvement of up to $2\%$.

% we outperformed the state-of-the-art reported PCC \cite{JIM} that uses Transformer model in a multi-task setting with up to 1.7\%
% outperforms the multi-task training which is considering words, utterance, fluency and other information along with phoneme-unit by. Thus indicating the supremacy of the SpeechBlending augmentation technique. 

\paragraph*{Effectiveness of the Masks: } We assess the effectiveness of each standalone mask incorporated in the SpeechBlender for creating different mispronunciation instances. Table \ref{tab:resuts_2} shows that the smooth blending masks (Smooth Overlay and Smooth-Gaussian Overlay) create more practical variation in mispronunciation and accented phonemes than their counter-part. When compared directly with the `Cut/Paste' augmentation mask, our blending mask also shows its efficacy, as only using 10K of augmented data generated by Smooth Overlay masking shows a relative improvement of 4\%. 

% We compared the following five experiments: 1)Training our proposed architecture on the official training data from Speechocean762 dataset; 2)Training on additional text-augmented data (additional 20K of accented phoneme pronunciations and 1K of totally mispronounced phoneme); 3)Training on additional GOP-augmented data (additional 20K of accented phoneme pronunciations and 1K of totally mispronounced phoneme); 4)Training with augmented data using SpeechBlender module (20k of accented phoneme pronunciations generated equally distributed over four proposed masking techniques: Smooth Overlay ($\lambda = 0.5$), CutMix, Smooth Concatenation and the Smooth-Gaussian Overlay, and an additional 1K of totally mispronounced phoneme data using cut/paste); 5)Training using the same augmented data used in experiment 4 and the original training set. We show all results in Table \ref{tab:resuts_1}. 

% For the proposed augmentation technique, it can be found that the additional 21K of data using SpeechBlender module improves the pearson correlation score from 0.58 to 0.61, with an important decrease in MSE from 0.090 to 0.085. With the same amount of additional augmented data, Our proposed SpeechBlender-based augmentation outperforms GOP-based augmentation and text-based augmentation techniques. With training LSTM on the additional SpeechBlender data outperforms the training on multi-tasks learning\cite{JIM} with additional 7 scores related to word and sentence pronunciation assessment under the same experimental setting. 

% In table \ref{tab:results_2}, different additional 5K of augmented data of accented and aberrant phonemes using different masks are shown. We noticed that for each proposed mask, training on additional 5K of augmented data using this mask outperforms the training on the original tarining set. SmoothOverlay with $\lambda = 0.5$ outperforms all other proposed mask augmentation technique.

% In table \ref{tab:results_3}, we compared our proposed data augmentation technique to create new totally mispronounced data with the baseline method cut/paste...

\begin{table} [!ht]
\centering
\arrayrulecolor{black}
\begin{tabular}{!{\color[rgb]{0,0,0}} l|l|l} 
\arrayrulecolor{black}\hline
\textbf{Training Dataset}                      & \textbf{PCC} & \textbf{MSE}                                           \\ 
\arrayrulecolor{black}\hline\hline
\multicolumn{3}{c}{\textbf{Baselines}}                                                                                  \\ 
% \arrayrulecolor{black}
\hline\hline
\textit{Original}                     &     0.58         &     0.090 \\   
\hline 
\textit{+ LSTM Multi-task Learning \cite{JIM}}    &     0.59         &     0.089                                                   \\ 
\hline 
\textit{+ Transformer Multi-task Learning \cite{JIM}}    &     0.61         &     0.085                                                   \\ 
\hline\hline
\multicolumn{3}{c}{\textbf{ Augmentation Baselines}}                                                                                  \\ 
\hline\hline
\textit{+ Text-augmentation}            &       0.59       &                  0.092                                     \\ 
% \arrayrulecolor{black}
\hline
\textit{+ GOP-augmentation}             &     0.59         &                    0.090                                    \\ 
% \arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-3}
\hline\hline
\multicolumn{3}{c}{\textbf{Our Proposed Augmentation Method}}                                                                              \\ 
% \arrayrulecolor{black}\hline
\hline\hline
% \arrayrulecolor{black}\hline
\textit{+ SpeechBlender-Aug} &         \textbf{0.63}     &                 \textbf{0.085} \\ \hline

\end{tabular}

\caption{Reported phoneme-level PCC and MSE on Speechocean762 test data}
\vspace{-0.4cm}
\label{tab:results_1}
% \arrayrulecolor{black}
\end{table}






\begin{table} [!ht]

\centering


\scalebox{1.0}{
\arrayrulecolor{black}
\begin{tabular}{!{\color[rgb]{0,0,0}} l|l|l} 
\arrayrulecolor{black}\hline
\textbf{Augmentation Mask}                      & \textbf{PCC} & \textbf{MSE}                                           \\ 
\arrayrulecolor{black}\hline\hline
\multicolumn{3}{c}{ \textit{Mask creating accented phoneme class, $\hat{y}=1$}}                                                                                  \\ 
\hline\hline

\textit{Smooth Overlay ($\lambda = 0.5$)}               &      \textbf{0.62}       &               \textbf{0.086}                                        \\ 
\hline
\textit{CutMix}                       &        0.59      &                   0.088                                     \\ 
\hline
\textit{Smooth Concatenation}         &      0.59        &              0.089                                          \\ 
\hline
\textit{Smooth-Gausian Overlay}       &      0.60        &   0.088\\
\hline
\textit{Smooth Overlay ($\lambda = 0.6$)}       &      0.61        &    0.087\\
\hline\hline
\multicolumn{3}{c}{ \textit{Mask creating mispronounced phoneme class, $\hat{y}=0$}}                                                                                  \\ 
\hline\hline
\textit{Cut/Paste}                         &         0.58    &                0.104                                        \\ 
\arrayrulecolor{black}\hline
\textit{Smooth Overlay ($\lambda = 0.1$)}               &      0.56       &                0.096                                    \\ 
\hline
\textit{Smooth Overlay ($\lambda = 0.2$)}       &      \textbf{0.58}        &    \textbf{0.092}\\\hline

\end{tabular}
}
\caption{Reported phoneme-level PCC and MSE on Speechocean762 test for different augmentation mask by adding additional \textbf{10K augmented phoneme} to the training dataset}

\vspace{-0.5cm}
\label{tab:resuts_2}
% \arrayrulecolor{black}
\end{table}


\subsection{AraVoiceL2 dataset:}
% \paragraph*{Effectiveness on AraVoiceL2: }  

We report the effectiveness of the SpeechBlender framework on the Arabic AraVoiceL2 testset. Due to the inadequacy of an effective Arabic acoustic model at the phoneme level, we focus our analysis solely on the grapheme level. As shown in Table \ref{tab:results_5}, our proposed augmentation technique achieve 4.63\% improvement in F1-score on AraVoiceL2 testset, it outperforms outperforms Text-augmentation and GOP-augmentation with 1.98\% and 1.44\% respectively. 

% , we followed a similar approach to Speechocean765 as shown in Figure \ref{fig:data_aug_pipeline}, which included creating a directory of pronunciation speech using AraVoiceL2 trainset , Arabic acoustic model \cite{} for force alignment, a close phoneme pair dictionary extracted from \cite{}. 




\begin{table} [!ht]
\centering
\arrayrulecolor{black}
\scalebox{0.85}{
\begin{tabular}{!{\color[rgb]{0,0,0}} l|l|l|l} 
\arrayrulecolor{black}\hline
\textbf{Training Dataset}                      & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score}                 \\ 
\arrayrulecolor{black}\hline\hline
\multicolumn{3}{c}{\textbf{Baselines}}                                                                                  \\ 
% \arrayrulecolor{black}
\hline\hline
\textit{Original}                     &     61.72\%          &     53.78\% &  55.37\% \\   
\hline\hline
\multicolumn{3}{c}{\textbf{ Augmentation Baselines}}                                                            \\ 
\hline\hline
\textit{+ Text-augmentation}            &       60.08\%      &       56.57\% & 58.08\%         \\ 
% \arrayrulecolor{black}
\hline
\textit{+ GOP-augmentation}             &    59.26\%      &       57.98\% & 58.56\%                                 \\ 
% \arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-3}
\hline\hline
\multicolumn{3}{c}{\textbf{Our Proposed Augmentation Method}}                                                                              \\ 
% \arrayrulecolor{black}\hline
\hline\hline
% \arrayrulecolor{black}\hline
\textit{+ SpeechBlender-Aug} &      60.33\%      &       \textbf{59.69}\% & \textbf{60.00}\%      \\ \hline

\end{tabular}
}
\caption{Reported Grapheme-Level Precision, Recall and F1-score on AraVoiceL2 Testset}
\vspace{-0.4cm}
\label{tab:results_5}
% \arrayrulecolor{black}
\end{table}


Our study indicates that the SpeechBlender framework is not only effective for English but also for Arabic at the grapheme-level.

% \begin{table}
% \label{tab:resuts_3}
% \centering
% \caption{Reported phoneme-level scores on testing dataset using different masking  used to create \textbf{totally mispronounced phoneme}.}

% \arrayrulecolor{black}
% \begin{tabular}{!{\color[rgb]{0,0,0}} l|l|l} 
% \arrayrulecolor{black}\hline
% \textbf{Training Dataset}                      & \textbf{PCC} & \textbf{MSE}                                           \\ 
% \arrayrulecolor{black}\hline
% \multicolumn{3}{c}{ \textbf{Per Mask}}                                                                                  \\ 
% \hline
% \textit{Original + Cut/Paste}                         &         0.55    &                0.104                                        \\ 
% \arrayrulecolor{black}\hline
% \textit{Original + Smooth Overlay ($\lambda = 0.1$)}               &      \textbf{0.56}       &                \textbf{0.096}                                      \\ 
% \hline
% \textit{Original + Smooth Overlay ($\lambda = 0.2$)}       &      0.58        &    \textbf{0.092}\\

% \end{tabular}
% \arrayrulecolor{black}
% \end{table}



% Training with additional data using the proposed data augmentation techniques 'SpeechBlender Box', we outperform swaping based baselines, GOP-augmentation technique and text-augmentation technique. An additional 21K phonemes generated using SpeechBlender Zero-Shot outperforms the LSTM model that was trained on mutli-learning task scheme (with additional 7 scores related to word, sentence assessment tasks).




% \label{sec:results}
% \subsection{Text-based Augmentation}

% \paragraph*{Key Observation:} Using SpeechBlender augmentation pipeline we observed improved performance compare to no-augmentation, multi-task learning secnation, text-augmentation, and GOP-augmentation setting. We observed the `Cut/Paste' method be it in text-, feature- or raw-audio domain is not as efficient as our fine-grained linear interpolation technique. We observed with blending the signals, we can generate new positive error classes instead of reusing samples from the data itself. Our method shows, without using any error labels from the original data, we are able to generate new error samples and improve the performance. The different masks included in the pipeline allows variations in transition and style of errors. Thus making it more efficient

% - +0.03 whereas 3M paper have added many geatures hubert wavlm, energy and many others to get +0.03 in terms of CORRELATION. 

% * -0.006 in MSE, compared to 3M who got -0.002.
% * need to report other augmentations techniques (the one with clustering) they got +0.3 in F1-score. 

%  the model would tend to output the prior phonemes and ignore the learn‘s mispronunciation, i.e., higher accuracy and lower recall, because the prior phoneme sequences were fed into the model, the most of which is negative samples, i.e., the number of negative samples is high and the number of positive samples is less, which leads to the model preferring to output canonical phonemes.

==> sections/introduction.tex <==
\section{Introduction} 
\label{sec:intro}

% The success of Deep  neural  networks (DNN) in speech technology, such as speech recognition, speech translation systems among others \cite{},  are driven by different networks structure \cite{}, with sophisticated training paradigm \cite{} as well as availability of high computational power \cite{}. 
% However, such success are not easily transferable to the tasks like Mispronunciation detection and diagnosis (MDD) system due to lack of a large amount of reliable training data. 

With the advent of globalization, more people are now inclined towards multilingualism. Such a shift in interest promotes the demand for the computer-aided pronunciation training (CAPT) system to language learning applications \cite{CAPT,CAPT_2}. The CAPT system potentially exploits the advancement of speech technology along with curriculum management and learner assessment among others. Mispronunciation detection (MD) and diagnosis system -- a crucial component of the CAPT -- detects the mispronunciation in an L2 learner‘s speech and highlights the error to give effective feedback. 
% Therefore, training such model need fine-grained human-annotated training data labeling the correctness of the each pronounced phoneme. As a result, such annotated data set are quite scare and often contain uneven positive class labels.\footnote{In case of MDD, the positive class represents -- missed, mispronounced or accented phonemes, and the negative classes are good pronounced phonemes.}

% To overcome the dependency on annotated data, 
%Over years, 
Researchers studied many methods to assess pronunciation quality. A majority of these methods use 
pre-trained automatic speech recognition (ASR) systems to either \textit{(i)} pinpoint the mismatch between the aligned ASR output sequence with the reference; or \textit{(ii)} utilize the log-posterior probability from the ASR to compute variants of the goodness of pronunciation (GOP) scores \cite{GOP_WITT,GOP_1,GOP_2} to asses pronunciation.
One successful line of research treated the mispronunciation detection as a regression, or a classification task \cite{transfer_}. Using deep learning, the network is either trained in an end-to-end manner \cite{non_ASR,non_ASR_2,non_ASR_3,DNN_3} or built upon the computed GOP features from the pre-trained ASR \cite{JIM,JIM_asr_BASED,likeJIM_asr,3M} to detect errors. These approaches are heavily dependent on the availability of a large amount of manually annotated datasets for the target demographic L2 speakers. However, such annotated datasets are scarce and often contain uneven positive class labels.\footnote{In the case of MD, the positive class represents -- missed, mispronounced, or accented phonemes, and the negative classes are good pronounced phonemes.}

% The mismatch between the aligned ASR output sequence with the reference are used to pinpoint mispronunciation. Moreover, researchers have entail the log-posterior probability to compute variants of goodness of pronunciation GOP \cite{GOP_WITT,GOP_1,GOP_2} score to asses pronunciation. %This method and its variants \cite{GOP_WITT,GOP_1,GOP_2} achieve a promising performance on mispronunciation detection.
% On the other hand, with a small amount of annotated training data, a significant jump in performance is observed when 
% The researchers have also treated the mispronunciation detection as a regression or a classification task \cite{transfer}. Using deep learning architecture, the network is either trained in an end-to-end manner \cite{non_ASR,non_ASR_2,non_ASR_3,DNN_3} or built upon the computed GOP features from the pre-trained ASR \cite{JIM,JIM_asr_BASED,likeJIM_asr,3M} to detect errors. Such design choice, despite showing high performance, heavily depend on the availability of a large amount of manually annotated dataset for the target demographic L2 speakers. As a result, such annotated data set are quite scare and often contain uneven positive class labels.\footnote{In case of MDD, the positive class represents -- missed, mispronounced or accented phonemes, and the negative classes are good pronounced phonemes.}


Data augmentation techniques are proven to be quite effective in overcoming scarcity in MD. Techniques involved (\textit{i}) modifying the canonical text with mismatched character pair keeping its original word-level speech intact \cite{non_ASR_3}; (\textit{ii}) using Text-To-Speech to synthesize `incorrect stress' samples along with modified lexical stress \cite{l2_GEN_SSL}; (\textit{iii}) using a mixup technique, in feature space -- based on phone-level GOP pool to design word level training data \cite{mixup}; and (\textit{iv}) using error distance of the clustered self supervised learning model embedding to replace the phoneme sound with another close sound unit \cite{ssl, ssl_2}. These techniques are heavily motivated by the `Cut/Paste' approach. However, the L2 learners' pronunciation is highly affected by their native phoneme set \cite{L2_effect,l2_arctic}, which makes such mixup -- Cut/Paste augmentation methods less efficient.

%The aforementioned techniques simulate mispronunciation errors by finding a target phoneme unit, in a different -- text, feature or audio space, and use it to replace the current unit. However, the L2 learners' pronunciation is highly affected by their native phoneme set \cite{L2_effect,l2_arctic} and `Cut/Paste' approach reuses the available information without generating any new feature variation in phoneme level. Thus making such mixup -- Cut/Paste augmentation methods less efficient.
%  However, as the L2 speech learning theory \cite{} suggests

%In this study, we introduce \textbf{SpeechBlender} -- a simple fine-grained data augmentation pipeline for generating mispronunciation errors in low-resource settings. The SpeechBlender framework linearly interpolates raw input signals utilizing different masks and mixing factors, allowing modification of different regions of a target phoneme. Moreover, the proposed framework generates new training samples using only good pronunciation units and thus capable of generating MD training data from any native/non-native speech datasets. 

%We show the effectiveness of the proposed augmentation framework over text- and GOP-based augmentation techniques using a significantly faster non-autoregressive LSTM \cite{lstm} model for phoneme-level MD task. We compare the performance of different masks -- such as Smooth Overlay, Smooth Concatenation, CutMix, and Smooth Gaussian Overlay -- in the SpeechBlender and show its efficacy over the well-known Cut/Paste technique. We present our results using a well-establish publicly available MD dataset, Speechocean762 \cite{speechocean}. While the proposed technique is studied for a specific task (MD) in this paper, the SpeechBlender can be broadly applicable as an augmentation technique for most sequence labeling such as accented ASR or classification task with audio/speech as input.

In this study, we introduce SpeechBlender – a novel fine-grained data augmentation pipeline for generating mispronunciation errors using only good pronunciation units in low-resource settings. Our method can generate MD training data from any native/non-native speech dataset. Our framework linearly interpolates raw input signals utilizing different masks and mixing factors, allowing modification of different regions of a target phoneme\footnote{Presence of a few or zero pronunciation mistakes in the training data.}. While the proposed technique is studied for mispronunciation detection, the SpeechBlender can be broadly applicable as an augmentation technique for most sequence labeling such as accented ASR or classification task with audio/speech as input.
Our contributions are:
\vspace{-0.1cm}
\setlength\itemsep{-0.5em}
\begin{enumerate}[label=(\alph*)]
\item Introduce the SpeechBlender, a fine-grained data augmentation pipeline capable of smoothly modifying regions of phonetic unit to generate erroneous pronunciation; 
\item Show the effectiveness of the proposed method over text-based and GOP-based augmentation;
\item Analyse the performance of different masks in the SpeechBlender and compare it with cut/paste signal approach;
\item Release the code and recipe for the SpeechBlender augmentation.\footnote{The code will be shared upon paper acceptance.}
\end{enumerate}


% In this paper, we are introducing a new fine-grained data augmentation pipeline 'SpeechBlender' to generate erroneous pronunciation by smoothly modifying phonetic regions, and we are showing its effectiveness over traditional text-, GOP-based data augmentation techniques and cut/paste signal approaches. SpeechBlender augmentation module is publicly available \footnote{The code will be shared upon paper acceptance.}.



% % To put in rs
% Data Augmentation and other regularization efforts are proved to be effective in such scenarios \cite{}. Many augmentation methods are proposed to modify the shape or property of the signal \cite{} and can be applied either in time or frequency axes. Techniques like vocal tract length perturbation, speed perturbation \cite{}, pitch adjustment \cite{}, noise addition \cite{}, SpecAugment \cite{} and variation of speech mixing \cite{} are applied successfully for Speech Recognition Systems, Audio classification among others.


% ### What this paper is about

% ### Motivation and Novelty

% ### List contribution
% -- new augmentation technique -- zero/few shot, linguistically motivated (independent of the task in hand)
% -- finegrained data aug
% -- pipeline/code release
% -- data release








% Notes extra motivations:

% -- text is easy to aug but does not generate much variation
% -- generating feature/GOP space aug like [] is interesting however wont be able to use in asr-independent models


==> sections/methodology.tex <==


\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{figures/pipeline_speechblender4.png}
\caption{Overview of the SpeechBlender, a fine-grained data augmentation pipeline, for zero-shot mispronunciation class generation. $U_C$: input speech utterance for candidate phoneme; $U_D$: selected speech utterance for donor phoneme; $x_C(T)$, $x_D(T)$ candidate and donor phoneme frames of length $T$ and $L$ respectively; $\hat{x}$ is the resultant augmented phoneme.}
\label{fig:data_aug_pipeline}
\end{figure}

\section{Methodology} 
\label{sec:method}

% %-- a fine-grained data augmentation pipeline, for generating mispronunciation classes in a low-resource settings.\footnote{Presence of a few or zero erroneous pronunciation examples in the data.} 
% %how many times do we define speechblender?!
% %From the canonical phoneme sequence of an input utterance $U_C$, 
% $U_C$ is an input utterance comprised of a canonical phoneme sequence.
% % Good pronounced phonemes are selected as \textbf{augmentation candidates}. 
% For each candidate unit, we pick a \textbf{donor phoneme} using a \textbf{close phoneme-pair dictionary} and choose another utterance, $U_D$ as a source signal of the selected donor phoneme. 
% Good pronounced phonemes 
% MFCC features for the $U_C$ and $U_D$ and obtain the corresponding phoneme time boundary using a publicly available pre-trained ASR. 
Figure \ref{fig:data_aug_pipeline} shows an overview of the SpeechBlender. $U_C$ represents an input utterance consisting of a sequence of canonical phonemes. For candidates phonemes selected from $U_C$, we consult a \textbf{close phoneme-pair dictionary} and select a \textbf{donor phoneme}. We select another utterance, $U_D$, that features the donor phoneme being pronounced accurately. This selected utterance, $U_D$, serves as a source signal for the donor phoneme.

We obtain the alignments of the utterances $U_C$ and $U_D$ using a pre-trained ASR, and get the corresponding phoneme time boundaries. Using the start and end boundary of the candidate, $x_C$,  and donor, $x_D$, phoneme, we select the speech frames and apply augmentation with the SpeechBlender. We then replace the candidate phoneme $x_C$ with the augmented phoneme frames $\hat{x}$ in the candidate utterance $U_C$.

% \subsection{Donor Unit Selection Module}
% \todo{@Yassine: Please re-write the module following a uniform terminology}
% Using the pretrained ASR model with KALDI librispeech recipe:
% \begin{itemize}
%   \item All training utterances were decoded at the phoneme level.
%   \item Training acoustic features were forced aligned with the canonical phonetic transcription using Viterbi alignment.
% \end{itemize}

% \subsection{Good Pronunciation Speech Directory}

% \subsubsection{Close Phoneme Pair Dictionary}
% All phonemes that were decoded correctly by the pretrained ASR acoustic model, and were judged by experts annotators as a good pronunciation
% , which we call the good pronunciation phoneme dictionary. 

% The `close phoneme pair dictionary' is designed to give a list of confused phonemes associated with the candidate phoneme.
\subsection{Close Phoneme Pair Dictionary}
%The `close phoneme pair dictionary' is designed to 
We randomly select a donor phoneme from a list of confused phonemes associated with the candidate phoneme. For English, the dictionary is constructed using 
% the Speechocean762 \cite{speechocean} and
L2-ARCTIC \cite{l2_arctic} confusing pairs matrix, and using the Speechocean762 \cite{speechocean} training set, and for Arabic, a similar dictionary was constructed using \cite{algabri2022mispronunciation} confusion pairs matrix. The entries are selected by analysing the confused phoneme pairs of speaker's pronunciation using ASR errors like substitution along with human annotation labels. Some examples of close phoneme pairs are presented in Table \ref{tab:examples_phoneme_pairs}.

% Once we get our donor, we randomly select another utterance from the training data which contain our donor phoneme. We then use 






% We analysed the substitution errors by the ASR model 
% % with the score assigned by expert annotators was less than 2, e.g accented and wrong pronunciations,
% ....
% % due to accentented , in addition to the many frequent mispronunciation 
% all phoneme from training data that were decoded incorrectly from the ASR model, and for which the score assigned by expert annotators was less than 2, e.g accented and wrong pronunciations, and all frequent confused pairs were stored in the dictionary. In order to make our confusing pairs phoneme more generalized, an additional amount of misconfusing phonemes were taken from L2-ARCTIC statistics, in which many frequent mispronunciation of different speakers with different L1-languages were reported.


% we have analyzed results, filtered good pronounced phoneme segment. All phonemes units that were decoded correctly from the ASR and was scored as a good pronunciation from the expert annotators were stored in a dictionary

\begin{table}[!ht]
\centering
\scalebox{0.9}{
\begin{tabular}{c} 
 \hline
 Close Phoneme Pairs (Confused \%) \\
 \hline\hline
 $SH \Leftrightarrow S$ (76\%), $V \Leftrightarrow F$ (44\%) ,  $NG \Leftrightarrow N$ (43\%), \\  $IY \Leftrightarrow IH$ (33\%),
 $Z \Leftrightarrow S$ (77\%) \\
 \hline
\end{tabular}
}
\caption{Examples of entries in Close Phoneme Pair Dictionary, with their \% of confusion.}
\label{tab:examples_phoneme_pairs}
\vspace{-0.2cm}
\end{table}

% \begin{table}[!ht]
% \centering
% \begin{tabular}{c|c} 
%  \hline
%  Close Phoneme Pairs & \% Confused \\
%  \hline\hline
%  $SH \Leftrightarrow S$  & 76\% \\ 
%  \hline
%  $V \Leftrightarrow F$ & 44\%  \\
%  \hline
%  $NG \Leftrightarrow N$ & 43\% \\
%  \hline
%  $IY \Leftrightarrow IH$  & 33\% \\
%  \hline
%  $Z \Leftrightarrow S$ & 77\% \\
%  \hline
% \end{tabular}
% \caption{Examples of entries in Close Phoneme Pair Dictionary, with their \% of confusion.}
% \label{tab:examples_phoneme_pairs}
% \end{table}

% To create new utterances, we parse a random audio X from the training set to the augmentation pipeline. First, we select randomly a phoneme ph1 that was scored 2 (correct pronunciation) from the expert annotators, we chose randomly a confusion pair phoneme ph2 from the confusion pairs dictionary. We select randomly from the good pronounciation phoneme dictionary a phoneme segment in which ph2 was pronounced correctly. we parse the ransom audio X to our pretrained ASR model to get alignment. Furthemore we augment using smoothMix function (ph1,ph2), and we end up with a new phnew (accented phoneme). We have proposed two SmoothMix function to generate new sounding phonemes, we associate to all this new generated phonemes a score of 1. From speechOcean765 annnotation guideline, an accented pronunciation or non-perfect pronuncoation is scored 1


% \subsubsection{Good Pronunciation Phoneme Directory}

% Using the pretrained ASR acoustic model on Librispeech, we get the forced alignment at the phoneme level, matching the phoneme with its corresponding timestamp from the corresponding audio. 

% % \todo{TODO: How the region are selected ??}
% \todo{TODO: Donor Phoneme selection ??}

\subsection{Pre-trained ASR and Alignment Module}
\label{ssec:asr}
We align the acoustic frames with the corresponding reference phoneme to obtain the start and end timestamps. For the force alignment, 
we employ the Hidden Markov Model-Time Delay Neural Network (HMM- TDNN)\footnote{https://kaldi-asr.org/models/m13} trained on Librispeech corpus as the acoustic model for SpeechOcean762 dataset alignment, and we used a CS-AR acoustic model ... for AraVoiceL2 alignment. Both acoustic models are trained using Kaldi \cite{kaldi}. 



% The alignment information of each phone and frame is get by force alignment using HMM-DNN (nnet3) model trained by speech recognition toolkit Kaldi [31].

\begin{figure*} [!ht]
\centering
\vspace{-0.4cm}
\includegraphics[width=0.8\textwidth]{figures/masks2.png}
\vspace{-0.5cm}
\caption{Comparison of the different masks used in the SpeechBlender augmentation framework. $x_C$ represent candidate phoneme (with length $T$) in the good data, augmented with the donor phoneme $x_D$ (length =$L$). 
$\mu$: the center-point; $R$: the number of regions the mask is divided into; $W$: list of widths of the regions; $\lambda$: the mixing factor in each region assigned in different augmentation scenarios given in (a) - (e). }
\label{fig:mask_types}
\end{figure*}

%%%Pseudo code here
\begin{algorithm}[h]
\label{algo:top}
\caption{SpeechBlender function}
\SetAlgoLined
\KwIn{Input phoneme frame sequences $x_C$ and $x_D$ where $x_C = \{f^1_C \cdots f^T_C\}$ and $x_D = \{f^1_D \cdots f^L_D\}$, where ($T$, $L$) are total frames in ($x_C$, $x_D$) respectively. $y_C$ represent the original output score assigned to the good phoneme.}
\KwOut{Augmented frame output sequences $\hat{x}$ and the corresponding label $\hat{y}$ of the output.}

\SetKwFunction{FMain}{Blender}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$x_C, x_D, y_C$}}{
        $\theta_{\hat{x}} \longleftarrow [ ]$ \Comment{Store augmented output per region}
        
        $\theta_{\hat{y}} \longleftarrow [ ]$ \Comment{Store corresponding partial output score}
        
        $mid \longleftarrow rand([1,4])$ \Comment{Mask template id}
        
        $\rho \longleftarrow get\_property(mid, len(x_C), len(x_D)) $ \Comment{Mask property}
        
        $ W, \Lambda \longleftarrow generate\_mask(\rho)$ 
        % \footnote{In case of MDD, the positive class represents -- missed, mispronounced or accented phonemes, and the negative classes are good pronounced phonemes.}

        
        \Comment{$W$: list of regional mask width, $\Lambda$: list of regional mixing factor values.}\
        % \Comment{}\
        % \Comment{$\hat{y}$: Output labels depending on the mixing factor}\
        % \Comment{$R$: list of frames divided in to regions, $\Lambda$: list of mixing factor for each region, $ \hat{y}$: generated output label  }
        
        
        % \Comment{$R \in  \{1, 2, 3\}$, $\Lambda \in [0-1]$, $ \hat{y} \in \{0, 1\}$ }
        
        
        \ForEach{$ w \in W$ and $ \lambda  \in \Lambda $}
        { 
        
        $x{_C^w}$$, x{_D^w}$ $\longleftarrow$ $x{_C}[w]$, $x{_D}[w]$$ 
        
        $\theta_{\hat{x}} \longleftarrow$ $\lambda \cdot x{_C^w}$ + $(1-\lambda ) \cdot x{_D^w}$ %\Comment{sorted list by weight}
        
        $\theta_{\hat{y}} \longleftarrow \lambda \cdot y{_C}
        }
        $\hat{x} \longleftarrow  Concat(\theta_{\hat{x}})$ %\Comment{join the regions generate augmented sample}
        
        $\hat{y} \longleftarrow   \left \lfloor \sum\theta_{\hat{y}}/len(\Lambda)\right \rfloor$
        
        
        \textbf{return} $\hat{x} , \hat{y} $ %\; 
}

\end{algorithm}
\vspace{-0.2cm}

\subsection{SpeechBlender}
Given the input frames of \textbf{good-phoneme candidate} $x_C$ and the donor-phoneme $x_D$, of length $T$ and $L$ respectively, our approach outputs the augmented phoneme $\hat{x}$ along with its corresponding output label $\hat{y}$. We first normalize the energy of $x_D$ to match $x_C$. Subsequently, we apply the SpeechBlender function, shown in Algorithm 1, with a selected mask templates.   

\paragraph*{Mask Templates:}  
We randomly select a mask template id, $mid \in [1-4]$. We then generate the property $\rho$ of the mask based on the $mid$, length of the phonemes $T$ and $L$. The property $\rho \in \{\mu, R, W, \Lambda\}$ is parameterized by the features of the mask including: \textit{(a)} the center-point $\mu = \frac{min(T,L)}{2}$; \textit{(b)} the number of regions $R\in \{1, 3\}$ the mask is divided into; \textit{(c)} along with a list containing all widths of the regions, $W$; and \textit{(d)} a list $\Lambda$, with its corresponding mixing factor with each value $\lambda \in [0-1]$. The width of each region is determined by the minimum frame length of inputs when both the input pair are considered with $\lambda > 0$. A $\lambda = 0$ for a signal represent a mixing weight of zero, meaning the full signal is blocked out.
Details of different mask templates along with their property, $\rho$, are presented in Figure \ref{fig:mask_types}.  

% For example, both the  $mid:2$-\textit{CutMix} and $mid:3$-\textit{SmoothConcatenation} (see Figure \ref{fig:mask_types}(c-d)) masks are composed of 3 regions with width -- $W_{mid:2} = \{ \frac{T}{3},  min(\frac{T}{3},\frac{L}{3}), \frac{T}{3} \}$ and $W_{mid:3} = \{ \frac{T}{3},  min(\frac{T}{3},\frac{L}{3}), \frac{L}{3} \}$ respectively.
%For the study, we opt for two types of Masks -- Rectangular (Figure \ref{fig:mask_types}(a)-(d)) and Gaussian (Figure \ref{fig:mask_types}(e)) masks. 


\paragraph*{Blending the Speech signals:} 
%, and its corresponding mixing factor $\lambda$in Algorithm \ref{algo:top}
The Given property $\rho$ of the mask, we generated the mask with its $W$ list and its corresponding $\Lambda$ list containing region-based $\lambda$ values. % and the corresponding new mispronunciation label $\hat{y}$.
Then for each regions in the mask, we multiply the $x{_C^w}$ and $x{_D^w}$ with $\lambda$ and $1- \lambda$ respectively (shown in Algorithm \ref{algo:top}) to create the regional augmented data $\theta_{\hat{x}}(.)$. We create the new augmented phoneme, $\hat{x}$ by concatenating all the $\theta_{\hat{x}}$ regional data.
The label $\hat{y} \in \{0,1\}$ of the augmented phoneme $\hat{x}$ is generated by averaging the regional label ($\theta_{\hat{y}} = \lambda \cdot y$). The $y$ is the value assigned to a good pronunciation of a phoneme.\footnote{These values are determined based on the original data annotation scheme. For this study, $y=2$.} The augmented output $\hat{y}=0$ represent the mispronounced or missing phoneme; whereas $\hat{y}=1$ represent the accented or aberrant phoneme unit. In our experiment, the regional augmented output is assigned $\theta_{\hat{y}} = 0$ if the mixing factor $\lambda<0.25$, otherwise it is assigned $\theta_{\hat{y}} = 1$.


% product of the mixing factor $\lambda$ along with the $y$ value assigned to the good pronunciation phoneme for e

% The number of width parameter of the mask, is determined as the value $mid$. 

% The rectangular masks are divided into regions, $R \in  \{1, 3\}$, with different region-specific mixing factors $\lambda \in [0-1]$. 
% For $R=3$

% The value of regions determine how the frames of the phoneme will be divided. For example, in case of mask 1, $mid:1$, we have 1 region with 1 mixing factor, whereas for $mid:3$, the phoneme-pairs are divided into three regions 

% Given a bag-of-masks (shown in Figure \ref{fig:mask_types})
% % can be seen as a variant of time masking technique, motivated by the SmoothMix, CutOut and CutMix technique in computer vision \cite{}. 
% % need to rewrite completely :::: todo for shammur
% The SpeechBlender is highly dependent on the type of mask, $M$ and the corresponding mixing factor $\lambda$. For the study, we opt for two types of Masks, $M$ -- rectangular and Gaussian masks as shown in Figure. 

% The choice of the mask and the $\lambda$ is one of the most crucial deciding factor for the 

% The property of the mask $\rho$ is highly dependent on the lengths of both the selected input phoneme $x_i$ and the augment-pair $x_j$. Generally the width of the mask is defined by these length 





% %%Talk about Energy normalization and then equation


% masking window property, $\rho$  and the corresponding mixing factor $\lambda$. For the study, we selected two types of masks, $M$ -- rectangular and Gaussian masks. The $\rho$ c

% % The generated property $\rho$ are based on the length of the selected input phoneme $x_i$ and the length of the selected candidate $x_j$ to augment.

% After selecting the phoneme 
% For the

% selecting the regions  in a phoneme along with the mixing factors to  transitioning Mask, M, generated based on the frame length, $T$ of the phoneme pairs $x_i^l, p_j^l$, we want to blend in. For the study, we used two different masks -- 
% where we mask a time portion to 

%%% Problem till here








% %%%% 
% One difficult of all pronunciation scoring models is the lack of accented and variants mispronunciation of phonemes in the training data. We have proposed three methods to generate more words and sentence samples with new generated accented phonemes.
% We increased the number of mispronounced phonemes using three main methods, overlaying two phonemes, soft-concatenation, and pitch-shift.

% The pipeline of our augmentation techniques has three main components, the pre-trained ASR model, the good pronunciation phoneme dictionary, and the confusion pairs dictionary. 



% \subsubsection{Overlay}
% Before overlaying the selected phonemes segments, we normalize the energy of ph2 segment, and then multiply by the energy of ph1. after we choose a blending mask G=0,5, and overlay the resulting segment.

% \[E_1 = Energy(X_{ph_{1}})\]
% \[E_2 = Energy(X_{ph_{2}})\]
% \[X^m_{ph_{1}} = X_{ph_{1}}*E_2/E_1\]
% \[Blending\;  mask:\;\; \; \; \;   G = 0.5\]
% \[=> X^{new} = G*X^m_{ph_{1}} + (1-G)*X_{ph_{2}}\]

% \subsubsection{Concatenation}
% Following the same steps of overlay smoothMix, for concatenationm instead of overlaying all phoneme segment, we belned the second half of ph1 and the first half of ph2 and we concotenate the resulting phoneme with the remaining part.
% we apply the energy moment exchange first. 
% \[E_1 = Energy(X_{ph_{1}})\]
% \[E_2 = Energy(X_{ph_{2}})\]
% \[X^m_{ph_{1}} = X_{ph_{1}}*E_2/E_1\]
% \[X^{tmp} = G*X^m_{ph_{1}}[/2:] + (1-G)*X_{ph_{2}}[:/2]\]
% \[=> X^{new} = Concatenate(X^m_{ph_{1}}[:/2],X^{tmp}, X_{ph_{2}}[/2:])\]

% \subsubsection{Additional Techniques}
% To make a fair comparison, we added another method to generate new sounding phones using pitch shifting, crop and paste, and exchange phonemes. For the phoneme randomly selected, 







\subsection{Baseline Augmentation Methods}
%We compare the performance of the SpeechBlender with text-level augmentation and GOP feature-level augmentation. % motivated by \cite{}.
\paragraph*{Text-based Augmentation}
For text-based phoneme data augmentation, we increase the number of error phoneme by altering the phoneme embedding from the canonical phoneme sequence. The candidate phoneme was replaced with a selected donor phoneme, using the same `close phoneme pair dictionary', when creating the canonical phoneme embedding space. An output label $\hat{y}=0$ is assigned when the candidate phoneme is swapped with a distant donor phoneme, for e.g., $SH \Leftrightarrow V$; whereas $\hat{y}=1$ is assigned for a close phoneme exchange such as $SH \Leftrightarrow S$.

% We increase the number of totally mispronounced phoneme by replacing phoneme embedding from the canonical phoneme sequence by another phoneme randomly selected from the list of all phonemes except phonemes that are close to the selected phoneme based on `close phoneme pair dictionary'.

\paragraph*{GOP-based Augmentation}
% Following the same technique as text augmentation, for GOP-based phoneme data augmentation, we increase the number of accented phoneme by altering the GOP features embedding. 
For GOP-based data augmentation, we first create a bag of GOP feature embedding for all good pronounced phonemes and grouped them by phoneme pairs using the same `close phoneme pair dictionary'. We then replaced the candidate phoneme, in the utterance with a donor phoneme GOP embedding randomly selected from the bag. We follow the same scoring scheme as text-augmentation for $\hat{y}$ labels.

% that stores GOP features embedding grouped by phoneme. We select randomly a candidate phoneme from the training utterance, and replace its GOP feature presentation with a selected donor phoneme GOP embedding selected randomly from the bag of GOPs. The donor phoneme is selected using the same `close phoneme pair dictionary'. 

% We increase the number of totally mispronounced phoneme by replacing GOP feature embedding by another phoneme GOP feature embedding randomly selected from the GOP embedding bag excluding embeddings of phonemes that are close to the selected phoneme based on `close phoneme pair dictionary'.




==> sections/related.tex <==
\section{Related Studies} 
\label{sec:related}

% \todo{Yassine}
A long story of research has been conducted to detect mispronunciation, the most known and dominant methods are Goodness-of-Pronunciation (GOP) scoring based and its variants. First, GOP was defined as the posterior probability of phoneme given the speech acoustics of the pronounced phonemes. Witt computed the formulated GOP using Gaussian Mixture model-hidden Markov Model (GMM-HMM), furthermore many improvements has been done to improve scoring of pronunciation, either by proposing new equivalent formulations of the first proposed GOP formula, or by improving the acoustic model quality, or by adopting deep learning models based scoring methods using acoustic features, and end-to-end scoring methods using CTC and self-supervised features. 

Zhang et al.[second] proposed a reformulation of GOP formula by calculating log-posteriors instead of posterior and scaled it to compute the overall phoneme score. Sweekar[third] derived a GOP formulation involving both posteriors and HMM state transition probabilities. [Context Aware] focused on phonetic context effects (such as liaison, omission, incomplete plosive sound, etc.), two additional factor were encoded, a transitional factor using entropy weight for frame-level posterior-probabilities, and a duration factor in the standard GOP. On the other hand, recent works showed that the pronunciation evaluation based on the score computed using Transformer have promising results and significant results, Jim's paper proposed multi-task learning Transformer based on GOP features with additional phonetic embeddings, another improvement has been conducted on the same Transformer scoring structure using Self-supervised Learning (SSL) Features (Wav2vec, HuBERT, WavLM), duration and energy features. 

Some recent works have proposed end-to-end models, from raw audio to pronunciation score. A fully end-to-end system  by aligning the audio with the phoneme sequences of the prior text inside the model through the attention mechanism has been proposed by {to site}, {SSL Audio} porposed two Transformer-Based architectures for mispronunciation detection (first structure using an encoder and decoder, second structure using wav2vec with contextual transformer block).  

Although these improvement in the GOP formulation and using end-to-end structure and attention mechanisms to improve the pronunciation scoring, little research focus was dedicated to investigate data augmentation techniques at phoneme level and word level that could improve the scoring technique. All proposed techniques and models were facing a problem of imbalance between good pronunciations samples and bad pronunciations specially accented samples. A simple text based augmentation technique by proposing three easy random replacement of phonemes using a set of close phonemes, vowels and consonants set based, and using confusing pairs based was proposed by ..., showed a significant increase of f1-score ... A recent work showed a significant improvement of word-level pronunciation scoring using mixup of deep acoustic features, the idea was inspired from the recent success of mixup on image classification. 


\paragraph*{Available Datasets}

\paragraph*{Goodness of Pronunciation}

\paragraph*{Architectures and Learning Methodologies}


==> sections/tmp.tex <==
One of the biggest challenges in designing mispronunciation detection models is the unavailability of labeled L2 speech data. To overcome such data scarcity, we introduce SpeechBlender -- a fine-grained data augmentation pipeline for generating mispronunciation errors. The SpeechBlender utilizes varieties of masks to target different regions of a phonetic unit, and use the mixing factors to linearly interpolate raw speech signals while generating erroneous pronunciation instances. The masks facilitate smooth blending of the signals, thus generating more effective samples than the `Cut/Paste' method. We show the effectiveness of our augmentation technique in a phoneme-level pronunciation quality assessment task, leveraging only a good pronunciation dataset. With SpeechBlender augmentation, we observed a 3% and 2% increase in Pearson correlation coefficient (PCC) compared to no-augmentation and goodness of pronunciation augmentation scenarios respectively for Speechocean762 testset. Moreover, a 2% rise in PCC is observed when comparing our single-task phoneme-level mispronunciation detection model with a multi-task learning model using multiple-granularity information.
